Tangent Schr\"odinger Bridge Matching: Learning Stochastic Transport with Mechanistic Sensitivities

Predicting how stochastic systems respond to changes in viscosity, reaction rates, or external forces requires costly simulations, motivating reusable learned models. Yet matching observed outcome distributions does not ensure accurate intervention responses. We introduce Tangent Schr\"odinger Bridge Matching (Tangent-SBM), which learns stochastic transports from endpoint observations and mechanistic sensitivities. It propagates parameter derivatives alongside trajectories and supervises them against supplied targets. For average-response targets, single-rollout squared error also penalizes response variability; our objective uses two independent rollouts to match the mean without this additional penalty. We establish conditions under which sensitivity accuracy bounds finite-change prediction error and decision regret. Across Gaussian, stochastic double-well, PDEBench reaction--diffusion, and stochastic Navier--Stokes systems, Tangent-SBM improves sensitivity and finite-change prediction over matched conditional-bridge baselines while maintaining comparable endpoint and distributional accuracy. Controls examine target correctness, response objectives, and simulator-budget allocation. To test decision usefulness, we evaluate calibrated viscosity selection in Navier--Stokes: Tangent-SBM reduces tracking error relative to taking no action on every evaluated task.

==> tables/full_splits.tex <==
\begin{table}[t]
\centering\small
\caption{Gaussian, Seen. Completed evaluation.}\label{tab:fullGaussianSeen}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.559\pm0.001$ & $1.000\pm0.000$ & $0.345\pm0.000$ \\
Conditional DSBM & $0.245\pm0.008$ & $1.048\pm0.007$ & $0.357\pm0.003$ \\
GSBM & $0.264\pm0.003$ & $1.051\pm0.001$ & $0.358\pm0.001$ \\
TSBM & $0.263\pm0.002$ & $1.051\pm0.002$ & $0.358\pm0.001$ \\
Tangent-SBM & $0.244\pm0.008$ & $0.035\pm0.004$ & $0.017\pm0.005$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{Gaussian, ID. Completed evaluation.}\label{tab:fullGaussianID}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.714\pm0.002$ & $1.000\pm0.000$ & $0.321\pm0.000$ \\
Conditional DSBM & $0.440\pm0.013$ & $0.866\pm0.003$ & $0.275\pm0.001$ \\
GSBM & $0.446\pm0.002$ & $0.865\pm0.001$ & $0.276\pm0.000$ \\
TSBM & $0.446\pm0.000$ & $0.865\pm0.001$ & $0.275\pm0.000$ \\
Tangent-SBM & $0.249\pm0.006$ & $0.050\pm0.005$ & $0.016\pm0.001$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{Gaussian, Near OOD. Completed evaluation.}\label{tab:fullGaussianNearOOD}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.511\pm0.004$ & $1.000\pm0.000$ & $0.237\pm0.000$ \\
Conditional DSBM & $0.481\pm0.036$ & $1.247\pm0.034$ & $0.249\pm0.004$ \\
GSBM & $0.505\pm0.003$ & $1.274\pm0.008$ & $0.252\pm0.002$ \\
TSBM & $0.504\pm0.005$ & $1.266\pm0.006$ & $0.250\pm0.001$ \\
Tangent-SBM & $0.245\pm0.007$ & $0.129\pm0.025$ & $0.021\pm0.004$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{Gaussian, Far OOD. Completed evaluation.}\label{tab:fullGaussianFarOOD}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $1.397\pm0.006$ & $1.000\pm0.000$ & $0.512\pm0.000$ \\
Conditional DSBM & $0.397\pm0.028$ & $0.664\pm0.008$ & $0.329\pm0.004$ \\
GSBM & $0.462\pm0.009$ & $0.681\pm0.008$ & $0.339\pm0.005$ \\
TSBM & $0.437\pm0.022$ & $0.672\pm0.011$ & $0.333\pm0.006$ \\
Tangent-SBM & $0.260\pm0.003$ & $0.137\pm0.026$ & $0.085\pm0.006$ \\
\bottomrule
\end{tabular}
\end{table}

\clearpage
\begin{table}[t]
\centering\small
\caption{Double well, Seen. Completed evaluation.}\label{tab:fullDoublewellSeen}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.392\pm0.004$ & $1.000\pm0.000$ & $0.092\pm0.000$ \\
Conditional DSBM & $0.174\pm0.007$ & $0.458\pm0.002$ & $0.040\pm0.001$ \\
Tangent-SBM & $0.168\pm0.003$ & $0.271\pm0.025$ & $0.022\pm0.003$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{Double well, ID. Completed evaluation.}\label{tab:fullDoublewellID}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.336\pm0.005$ & $1.000\pm0.000$ & $0.110\pm0.000$ \\
Conditional DSBM & $0.186\pm0.006$ & $0.341\pm0.030$ & $0.035\pm0.005$ \\
Tangent-SBM & $0.177\pm0.002$ & $0.249\pm0.022$ & $0.025\pm0.003$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{Double well, Near OOD. Completed evaluation.}\label{tab:fullDoublewellNearOOD}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.499\pm0.002$ & $1.000\pm0.000$ & $0.042\pm0.000$ \\
Conditional DSBM & $0.168\pm0.008$ & $1.205\pm0.223$ & $0.045\pm0.007$ \\
Tangent-SBM & $0.166\pm0.004$ & $0.303\pm0.005$ & $0.013\pm0.001$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{Double well, Far OOD. Completed evaluation.}\label{tab:fullDoublewellFarOOD}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.542\pm0.005$ & $1.000\pm0.000$ & $0.023\pm0.000$ \\
Conditional DSBM & $0.167\pm0.007$ & $2.549\pm0.299$ & $0.055\pm0.006$ \\
Tangent-SBM & $0.166\pm0.006$ & $0.984\pm0.216$ & $0.022\pm0.007$ \\
\bottomrule
\end{tabular}
\end{table}

\clearpage
\begin{table}[t]
\centering\small
\caption{PDEBench, Seen. Completed evaluation.}\label{tab:fullPDEBenchSeen}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.715\pm0.029$ & $1.000\pm0.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.648\pm0.033$ & $0.828\pm0.019$ & $0.833\pm0.016$ \\
GSBM & $0.923\pm0.024$ & $0.801\pm0.012$ & $0.805\pm0.010$ \\
TSBM & $0.906\pm0.015$ & $0.805\pm0.036$ & $0.808\pm0.035$ \\
Tangent-SBM & $0.624\pm0.072$ & $0.479\pm0.048$ & $0.493\pm0.049$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{PDEBench, ID. Completed evaluation.}\label{tab:fullPDEBenchID}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.612\pm0.034$ & $1.000\pm0.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.605\pm0.038$ & $0.847\pm0.054$ & $0.843\pm0.054$ \\
GSBM & $0.918\pm0.022$ & $0.786\pm0.009$ & $0.784\pm0.009$ \\
TSBM & $0.904\pm0.013$ & $0.789\pm0.027$ & $0.787\pm0.028$ \\
Tangent-SBM & $0.598\pm0.069$ & $0.508\pm0.045$ & $0.510\pm0.046$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{PDEBench, Near OOD. Completed evaluation.}\label{tab:fullPDEBenchNearOOD}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.740\pm0.036$ & $1.000\pm0.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.668\pm0.020$ & $0.882\pm0.022$ & $0.878\pm0.022$ \\
GSBM & $0.917\pm0.023$ & $0.847\pm0.011$ & $0.845\pm0.010$ \\
TSBM & $0.901\pm0.012$ & $0.847\pm0.013$ & $0.845\pm0.012$ \\
Tangent-SBM & $0.641\pm0.062$ & $0.490\pm0.048$ & $0.492\pm0.045$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{PDEBench, Far OOD. Completed evaluation.}\label{tab:fullPDEBenchFarOOD}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.853\pm0.032$ & $1.000\pm0.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.729\pm0.024$ & $0.864\pm0.065$ & $0.867\pm0.070$ \\
GSBM & $0.949\pm0.027$ & $0.888\pm0.007$ & $0.885\pm0.007$ \\
TSBM & $0.928\pm0.014$ & $0.901\pm0.060$ & $0.900\pm0.062$ \\
Tangent-SBM & $0.678\pm0.066$ & $0.547\pm0.044$ & $0.548\pm0.045$ \\
\bottomrule
\end{tabular}
\end{table}

\clearpage
\begin{table}[t]
\centering\small
\caption{SNS, Seen. Original MC16 response diagnostic; distinct from the pending MC1024 table.}\label{tab:fullSNSSeen}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.301\pm0.019$ & $1.000\pm0.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.267\pm0.048$ & $2.944\pm0.195$ & $2.872\pm0.182$ \\
GSBM & $0.231\pm0.017$ & $3.700\pm0.700$ & $3.637\pm0.698$ \\
TSBM & $0.178\pm0.003$ & $2.665\pm0.018$ & $2.587\pm0.031$ \\
Tangent-SBM & $0.266\pm0.026$ & $1.364\pm0.276$ & $1.393\pm0.307$ \\
SpreadBudget & $0.285\pm0.013$ & $3.826\pm0.419$ & $3.709\pm0.372$ \\
LocalBudget & $0.274\pm0.007$ & $3.096\pm0.455$ & $3.010\pm0.402$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{SNS, ID. Original MC16 response diagnostic; distinct from the pending MC1024 table.}\label{tab:fullSNSID}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.298\pm0.021$ & $1.000\pm0.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.265\pm0.047$ & $2.794\pm0.208$ & $2.429\pm0.158$ \\
GSBM & $0.227\pm0.017$ & $3.634\pm0.795$ & $3.207\pm0.768$ \\
TSBM & $0.176\pm0.002$ & $2.498\pm0.065$ & $2.185\pm0.059$ \\
Tangent-SBM & $0.265\pm0.028$ & $1.439\pm0.347$ & $1.291\pm0.354$ \\
SpreadBudget & $0.283\pm0.011$ & $3.649\pm0.332$ & $3.145\pm0.281$ \\
LocalBudget & $0.272\pm0.005$ & $2.929\pm0.403$ & $2.517\pm0.307$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{SNS, Near OOD. Original MC16 response diagnostic; distinct from the pending MC1024 table.}\label{tab:fullSNSNearOOD}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.299\pm0.016$ & $1.000\pm0.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.266\pm0.048$ & $4.993\pm0.284$ & $4.051\pm0.278$ \\
GSBM & $0.229\pm0.018$ & $5.665\pm0.696$ & $4.756\pm0.622$ \\
TSBM & $0.179\pm0.003$ & $4.452\pm0.175$ & $3.654\pm0.123$ \\
Tangent-SBM & $0.265\pm0.027$ & $2.048\pm0.227$ & $1.703\pm0.221$ \\
SpreadBudget & $0.286\pm0.011$ & $6.433\pm1.091$ & $5.225\pm0.852$ \\
LocalBudget & $0.275\pm0.004$ & $5.378\pm1.010$ & $4.329\pm0.805$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering\small
\caption{SNS, Far OOD. Original MC16 response diagnostic; distinct from the pending MC1024 table.}\label{tab:fullSNSFarOOD}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ & Finite change \\
\midrule
DSBM & $0.297\pm0.020$ & $1.000\pm0.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.260\pm0.047$ & $5.015\pm0.196$ & $4.938\pm0.257$ \\
GSBM & $0.230\pm0.017$ & $5.513\pm0.748$ & $5.498\pm0.692$ \\
TSBM & $0.177\pm0.002$ & $4.532\pm0.267$ & $4.448\pm0.230$ \\
Tangent-SBM & $0.259\pm0.027$ & $2.024\pm0.130$ & $1.992\pm0.181$ \\
SpreadBudget & $0.279\pm0.015$ & $6.441\pm1.138$ & $6.347\pm1.121$ \\
LocalBudget & $0.270\pm0.008$ & $5.407\pm1.061$ & $5.306\pm1.040$ \\
\bottomrule
\end{tabular}
\end{table}

\clearpage


==> tables/sns_id.tex <==
\begin{table}[t]
\centering\small
\caption{SNS ID comparison. Endpoint MC32 and finite-change MC16 are completed evaluations. The common-budget MC1024 derivative evaluation is pending; its values are not inferred from development diagnostics.}\label{tab:sns}
\begin{tabular}{lccc}
\toprule
Method & Endpoint & $E_J$ (MC1024) & Finite change \\
\midrule
DSBM & $0.298\pm0.021$ & $1.000$ & $1.000\pm0.000$ \\
Conditional DSBM & $0.265\pm0.047$ & \pending & $2.429\pm0.158$ \\
GSBM & $0.227\pm0.017$ & \pending & $3.207\pm0.768$ \\
TSBM & $0.176\pm0.002$ & \pending & $2.185\pm0.059$ \\
Tangent-SBM & $0.265\pm0.028$ & \pending & $1.291\pm0.354$ \\
\bottomrule
\end{tabular}
\end{table}

